Measurements of multiplicity fluctuations of identified hadrons in inelastic proton-proton interactions at the CERN Super Proton Synchrotron

Measurements of multiplicity fluctuations of identified hadrons produced in inelastic p+p interactions at 31, 40, 80, and 158~\GeVc beam momentum are presented. Three different measures of multiplicity fluctuations are used: the scaled variance $\omega$ and strongly intensive measures $\Sigma$ and $\Delta$. These fluctuation measures involve second and first moments of joint multiplicity distributions. Data analysis is performed using the Identity method which corrects for incomplete particle identification. Strongly intensive quantities are calculated in order to allow for a direct comparison to corresponding results on nucleus-nucleus collisions. The results for different hadron types are shown as a function of collision energy. A comparison with predictions of string-resonance Monte-Carlo models: Epos, Smash and Venus, is also presented.

==> sections/01-app.tex <==
\section{Strongly intensive measure $\Phi$}
\red{NA49 results are now available in $\Sigma$ and $\Delta$ so maybe remove $\Phi$ completely}


The first strongly intensive quantity $\Phi$ was
introduced in 1992~\cite{Gazdzicki:1992ri} and can be expressed via $\Sigma$:
\begin{equation}
\label{Eq:phi}
\Phi[a,b]=\frac{\sqrt{\langle N_a \rangle\langle N_b \rangle}}{\langle N_a+N_b \rangle}\cdot\left(\sqrt{\Sigma[a,b]}-1\right).
\end{equation}

\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{figures/phi_full}
				
\caption[]{
	The collision energy dependence of $\Phi[\pi,(p+\overline{p})]$,
	$\Phi[\pi, K]$ and $\Phi[(p+\overline{p}),K]$ in inelastic \pp interactions. 
	Results for all charged, positively and negatively charged hadrons are presented separately.
		The solid, dashed and dotted lines show predictions of \EposLong, \SmashLong and \VenusLong models, respectively. Statistical uncertainty is denoted with bar and systematic uncertainty is indicated with red band.
	 }
\label{fig:phi}
\end{figure*}

Figure~\ref{fig:phi} shows the results on $\Phi$ for 
pion-proton, pion-kaon and proton-kaon multiplicities
measured separately for all charged, positively
charged, and negatively charged hadrons produced in inelastic \pp collisions at 31--158~\GeVc beam momentum. 
The strongly intensive measures $\Sigma$ and $\Phi$ differ only by a selection of the reference value (one for $\Sigma$ and zero  for $\Phi$) and a normalization factor which involves mean multiplicities, see Eq.~\ref{Eq:phi}. $\Phi$ is presented here due to historical reasons, but only results for $\Sigma$ are discussed.


==> sections/06-analysis.tex <==
\section{Data analysis}\label{sec:analysis}


This section starts with a brief overview of the data analysis procedure and the applied corrections.

The analysis procedure consists of the following steps:
\begin{enumerate}[(i)]
	\item application of event and track selection criteria,
	\item determination of inclusive \dedx spectra,
	\item determination of moments of identified hadron multiplicity distributions with the Identity method,
	\item evaluation of corrections to the moments based on
	experimental data and simulations,
	\item calculation of the corrected moments and fluctuation quantities,
	\item calculation of statistical and systematic uncertainties.
\end{enumerate}  



Corrections for the following biases were evaluated and applied:
\begin{enumerate}[(i)]
	\item contribution of particles other than \emph{primary} (see below)
	hadrons produced  in inelastic \pp interactions,
	\item losses of primary hadrons due to measurement inefficiencies, 
	\item losses of inelastic \pp interactions due to the trigger and the
	event and track selection criteria employed in the analysis 
	%as well as losses of produced hadrons in accepted interactions
	%due to their decays and secondary interactions.
\end{enumerate}



The final results refer to identified hadrons 
produced in inelastic \pp interactions 
by strong interaction processes and in  electromagnetic
decays of produced hadrons. 
Such hadrons are referred to as \emph{primary} hadrons.


The analysis was performed in the kinematic acceptance limited by the detector geometry and 
the statistics of inclusive \dedx spectra. 
The acceptance is given in the form of two sets of tables:
\begin{enumerate}[(i)]
\item three-dimensional tables representing the high efficiency region of the detector,
\item two-dimensional tables defining the \dedx fit range.
\end{enumerate}
The acceptance tables can be found in Ref.~\cite{na61ParticlePopulationMatrix}.




